Incremental Deep Neural Network Learning using Classification Confidence Thresholding

Most modern neural networks for classification fail to take into account the concept of the unknown. Trained neural networks are usually tested in an unrealistic scenario with only examples from a closed set of known classes. In an attempt to develop a more realistic model, the concept of working in an open set environment has been introduced. This in turn leads to the concept of incremental learning where a model with its own architecture and initial trained set of data can identify unknown classes during the testing phase and autonomously update itself if evidence of a new class is detected. Some problems that arise in incremental learning are inefficient use of resources to retrain the classifier repeatedly and the decrease of classification accuracy as multiple classes are added over time. This process of instantiating new classes is repeated as many times as necessary, accruing errors. To address these problems, this paper proposes the Classification Confidence Threshold approach to prime neural networks for incremental learning to keep accuracies high by limiting forgetting. A lean method is also used to reduce resources used in the retraining of the neural network. The proposed method is based on the idea that a network is able to incrementally learn a new class even when exposed to a limited number samples associated with the new class. This method can be applied to most existing neural networks with minimal changes to network architecture.

==> OldSections.tex <==
\begin{comment} %Old Abstract
        Few environments are static in typical day-to-day experiences. Interpretation of data that is consciously known is forever changing and evolving. The majority of environmental aspects are often unknown, which feeds back to affect known interpretations of available data. Learning is a structural component of human behavior and requires a threaded connection between what is not currently known for fact and knowledge previously stored away. Modern neural approaches create environments that encompass the specifics of issues and naturally fail to incorporate the concept of new environmental changes. Reliance on the structure of data, the source of the data, and intention put forth by the environment creator, all limit the capabilities of applied neural networks. By forming an early plan of disposal for neural systems, there is an expected waste of previous knowledge and resources which has increasingly become more intensive to re-gather. From an initial neural network architecture and knowledge set, an incremental learning process reduces the need for re-learning and improves upon the accuracy of a network. Such a neural process also expects a combination of previously known and unknown data to be found during testing. This paper proposes an approach that can be implemented in current architectures to move models to use an incremental learning architecture. 
\end{comment}
        
\begin{comment} %Pieces of old introduction
        The process of learning can be described as the acquisition of skills through study and observation. From the moment they are born, humans are a prime example of entities that are capable to learn and gain knowledge. Over time sensory information through the human subconscious and environment-controlled communication allow for humans to learn and adapt in their environment. In general, training neural networks (NN) uses many concepts that relate to the psychology of human learning. Operant behavior, coined by \citep{skinner1937operant}, is behavior controlled by reward and consequence. A reward is given for the desired output, and in consequence of wrongful action, punishment is encountered to reduce the mistakes a subject makes. In the context of neural network training, this concept is heavily used. Imposing minimizations on mistakes and maximizations of desired output via loss functions is common among many neural architectures. Loss functions minimize or maximize an input to probabilistically produce the desired result. The groundwork of the loss function was introduced by \citep{laplace1820theorie} and exists in almost all modern NNs. Repeating the learning process allows for ongoing improvement which eventually can lead to an acceptable solution. 
        
        Much like humans, a neural network does not make all assumptions with one or two exposures to data. Knowledge is built by trial. An advantage of programmatically creating these systems allows for some hyperparameters of networks to change the natural behavior of data exposure. One example of this is the learning rate of an optimizer within a neural architecture. This parameter controls the overshoot of data optimization that can occur and prevent the assumption of unintentional functional mapping of input to output.
        %In human exposure, the brain acts in this way subconsciously. Humans act on survival, meaning that they do not forget what they have come to trust as truth, and at the same time, act in restraint to categorize a new action as correct and safe \citep{skinner1963operant}. 
        To further model the learning behavior in a NN training process, we must incorporate a mechanism to preserve the knowledge that is trusted, while allowing for the trials to discover new correct actions. 
\end{comment}
